Learning not to Regret

The literature on game-theoretic equilibrium finding predominantly focuses on single games or their repeated play. Nevertheless, numerous real-world scenarios feature playing a game sampled from a distribution of similar, but not identical games, such as playing poker with different public cards or trading correlated assets on the stock market. As these similar games feature similar equilibra, we investigate a way to accelerate equilibrium finding on such a distribution. We present a novel "learning not to regret" framework, enabling us to meta-learn a regret minimizer tailored to a specific distribution. Our key contribution, Neural Predictive Regret Matching, is uniquely meta-learned to converge rapidly for the chosen distribution of games, while having regret minimization guarantees on any game. We validated our algorithms' faster convergence on a distribution of river poker games. Our experiments show that the meta-learned algorithms outpace their non-meta-learned counterparts, achieving more than tenfold improvements.

==> Makefile <==
all: *.tex
	pdflatex main
	bibtex main
	pdflatex main
	pdflatex main

main: *.tex
	pdflatex main

clean:
	rm -f main.aux
	rm -f main.bbl
	rm -f main.bcf
	rm -f main.blg
	rm -f main.glg
	rm -f main.glo
	rm -f main.gls
	rm -f main.ist
	rm -f main.idx
	rm -f main.lof
	rm -f main.lot
	rm -f main.out
	rm -f main.log
	rm -f main.pdf
	rm -f main.run.xml
	rm -f main.*sbl
	rm -f main.*sym
	rm -f main.tex.bbl
	rm -f main.tex.blg
	rm -f main.toc
	rm -f main.mw
	rm -f *.cut

check:
	for file in *text; do \
	   aspell check $${file}; \
	done

